Learning to Recognize Actionable Static Code Warnings (is Intrinsically Easy)

Static code warning tools often generate warnings that programmers ignore. Such tools can be made more useful via data mining algorithms that select the "actionable" warnings; i.e. the warnings that are usually not ignored. In this paper, we look for actionable warnings within a sample of 5,675 actionable warnings seen in 31,058 static code warnings from FindBugs. We find that data mining algorithms can find actionable warnings with remarkable ease. Specifically, a range of data mining methods (deep learners, random forests, decision tree learners, and support vector machines) all achieved very good results (recalls and AUC (TRN, TPR) measures usually over 95% and false alarms usually under 5%). Given that all these learners succeeded so easily, it is appropriate to ask if there is something about this task that is inherently easy. We report that while our data sets have up to 58 raw features, those features can be approximated by less than two underlying dimensions. For such intrinsically simple data, many different kinds of learners can generate useful models with similar performance. Based on the above, we conclude that learning to recognize actionable static code warnings is easy, using a wide range of learning algorithms, since the underlying data is intrinsically simple. If we had to pick one particular learner for this task, we would suggest linear SVMs (since, at least in our sample, that learner ran relatively quickly and achieved the best median performance) and we would not recommend deep learning (since this data is intrinsically very simple).

==> texintrinsic.tex <==

\begin{figure}[!b]
\centerline{\includegraphics[width=0.45\textwidth]{figs/intrinsic.eps}}
\caption{Process of Box-counting Method to get Intrisic Dimensionality of Hyper Dimension dataset.}   
\label{fig:dimension}
\end{figure}



% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[]
% \caption{Summary of data distribution.}
% % \small
% \normalsize
% \begin{adjustbox}{max width=0.48\textwidth}
% \begin{tabular}{@{}cccccc@{}}
% \midrule
%  &  & \multicolumn{2}{c}{training set} & \multicolumn{2}{c}{test set} \\ \midrule
%  & Dataset & \begin{tabular}[c]{@{}c@{}}instance \\ counts\end{tabular} & \begin{tabular}[c]{@{}c@{}}actionable \\ ratio(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}instance \\ counts\end{tabular} & \begin{tabular}[c]{@{}c@{}}actionable \\ ratio(\%)\end{tabular} \\ \midrule
% \multirow{9}{*}{Projects} & Derby & 2479 & 8.67 & 2507 & 4.83 \\
%  & Mvn & 813 & 8.49 & 818 & 3.42 \\
%  & Lucence & 3259 & 36.88 & 3425 & 34.10 \\
%  & Phoenix & 2235 & 17.58 & 2389 & 14.36 \\
%  & Cass & 2584 & 14.82 & 2601 & 13.69 \\
%  & Jmeter & 604 & 24.83 & 613 & 23.65 \\
%  & Tomcat & 1435 & 27.80 & 1441 & 22.62 \\
%  & Ant & 1229 & 18.71 & 1115 & 4.84 \\
%  & Commons & 725 & 7.03 & 786 & 5.34 \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \label{table:distribution}
% \end{table}



\begin{algorithm}
\footnotesize
\begin{algorithmic}
\SetAlgoLined
\STATE{Import data from \texttt{Testdata.py}}
\STATE{$Input: sample\_num=n, sample\_dim=d$}

    \STATE{$Rs_{log} = start:end:step$}
    \STATE{ $Rs= np.exp(Rs_{log})$}
    \FOR{$R$ in $Rs$}
        \STATE{\# increasing the Euclidean radius}
        \STATE{$I = 0$}
        \STATE{\# count for pairwise samples within R}
        \FOR{$i,j$ in $combinations(data,2)$}
            \STATE{$d=distance(i,j)$}
            \IF{$d<R$}
                \STATE{$I \gets I+1$}
            \ENDIF
        \ENDFOR
        \STATE{$Cr=2*I/n*(n-1)$}
    \ENDFOR
    \STATE{$Crs.append(Cr)$}
    
    \FOR{$i$ in $step$}
    \STATE{$gradient=(Crs[i]-Crs[i-1])/(R[i]-R[i-1])$}
    \STATE{$GR.append(gradient)$}
    \ENDFOR
    \STATE{$Smooth(GR)$}
    \STATE{\# smooth the curve}
    \STATE{$intrinsicD \gets max(GR)$}
    \STATE{\# Estimate the intrinsic dimensionality}
    % \IF{$i\geq 5$} 
    %     \STATE{$i\gets i-1$}
    % \ELSE
    %     \IF{$i\leq 3$}
    %         \STATE{$i\gets i+2$}
    %     \ENDIF
    % \ENDIF 
\end{algorithmic}
\caption{Pseudo Code for Intrinsic Dimension by Box-counting Method}
\label{alg:intrinsic}
\end{algorithm}




\subsection{Intrinsic Dimension}

The intrinsic dimensionality (ID) of a representation refers to the minimum number of features necessary to capture the entire information present
in the representation
\cite{camastra2002estimating}.

Levina et al.~\cite{levina2005maximum} indicate that the reason any method works for high dimensions is that data embedded in high-dimensional format actually can be converted into a more 
compressed space without major information loss. Unnecessary high feature dimension not only burdens computational cost, also damage the generalization capability of the classifiers statistically~\cite{camastra2002estimating}. To cope with feature redundancy issue, many statistical procedures are proposed. The most famous one, PCA (Principal Component Analysis) has been proven efficient in linear transformation, which converts correlated features by orthogonal decomposition into a lower dimension (consisted of minimum number of linearly uncorrelated variables or principal components). However, as data in real world becomes increasingly sophisticated and non-linearly decomposable, traditional linear PCA methods tends to overestimate the dimensions of datasets. 
Nonlinear feature extraction methods is imperative to bridge the gap in estimating ID.  

Levina et al.~\cite{levina2005maximum} propose a fractal-based method and has now been widely used in astrophysics as a standard. 
% 
The intrinsic dimension of a dataset with \textit{N}
items is found by computing the number of items found at distance within radius \textit{r} (where \textit{r} is the Euclidean distance between two configurations) while varying \textit{r}. This is then normalized by the number of connections between k items to find the  expected number of neighbors at distance r. This can be written as:
%

\[ C(r) = \frac{2}{N(N-1)} \sum_{i=1}^N \sum_{j=i + 1}^N I (||x_i,x_j||<r) \]
\[where: I (||x_i,x_j||<r) = \left\{
    \begin{aligned}
    1, ||x_i,x_j|| < r \\
    0, ||x_i,x_j|| \ge r
    \end{aligned}
    \right. \]
    
%    
Given the dataset with k items and range of distances [r0 – rmax], we estimate the intrinsic dimensionality as the slope between ln(C(r)) and ln(r). The pseudo code of our methodology to estimate intrinsic dimensionality is illustrated in Algorithm~\ref{alg:intrinsic}.
% 

==> texoptions.tex <==
\begin{table}

%\captionsetup{font=footnotesize}
\caption{Options for Learners and preprocessors used in recent SE studies~\cite{ghotra2015revisiting,fu2016tuning,agrawal2018better,agrawal2018wrong} and from Scikit-learn~\cite{pedregosa2011scikit} for exploration of this work.
% While this list is incomplete, it does include many
% of the   hyperparameter optimizations being explored in the literature. 
}\label{tbl:options}
\footnotesize
 
\begin{tabular}{|p{.95\linewidth}|}\hline
\textbf{Learners:}  


\noindent
\bi
\item DecisionTreeClassifier(criterion=b, splitter=c, min\_samples\_split=a)
    \bi
   \item a, b, c= randuniform(0.0,1.0), randchoice([`gini',`entropy']), \newline randchoice([`best',`random'])
   \ei
\item RandomForestClassifier(n\_estimators=a,criterion=b,  min\_samples\_split=c)
    \bi
   \item a,b,c = randint(50, 150), randchoice(['gini', 'entropy']),\newline randuniform(0.0, 1.0) 
   \ei
\item SupportVectorMachine(kernal= a, penalty=b, gamma=c)
    \bi
    \item a,b,c=randchoice([`linear',`poly',`sigmoid']),randint(1,50),\newline randuniform(0.0,0.1)
    \ei 
% \item MultinomialNB(alpha=a) = randuniform(0.0,0.1)
% \item KNeighborsClassifier(n\_neighbors=a, weights=b, p=d, metric=c)
%     \bi
%     \item a, b,c  = randint(2, 25), randchoice([`uniform', `distance']), \newline randchoice([`minkowski',`chebyshev'])
%     \item if c=='minkowski': d= randint(1,15)  else:  d=2
%     \ei

\ei
\\\hline

{\bf Pre-processors for static warning analysis:} 

\bi 
\item StandardScaler
\item MinMaxScaler
\item MaxAbsScaler
\item RobustScaler(quantile\_range=(a, b)) =  randint(0,50), randint(51,100) 
\item KernelCenterer
\item QuantileTransformer(n\_quantiles=a,  output\_distribution=c, subsample=b)
    \bi
    \item a, b = randint(100, 1000), randint(1000, 1e5)
    \item c = randchoice([`normal',`uniform'])
    \ei
\item Normalizer(norm=a) = randchoice([`l1', `l2',`max'])
  
\item Binarizer(threshold=a) =  randuniform(0,100)
   
    \item SMOTE(a=n\_neighbors, b=n\_synthetics,  c=Minkowski\_exponent)
    \bi
    \item a,b = randit(1,20),randchoice(50,100,200,400)
    \item c = randuniform(0.1,5)
    \ei
\ei

 \\\hline
% {\bf Pre-Processors for Text mining:}  
 
% \bi
% \item CountVectorizer(max\_df=a, min\_df=b) = randint(100, 1000), randint(1, 10)
% \item TfidfVectorizer(max\_df=a, min\_df=b, norm=c)
%     \bi
%     \item a, b,c = randint(100, 1000), randint(1, 10), randchoice([`l1', `l2', None])
%     \ei
% \item HashingVectorizer(n\_features=a, norm=b)
%     \bi
%     \item a = randchoice([1000, 2000, 4000, 6000, 8000, 10000])
%     \item b = randchoice([`l1', `l2', None])
%     \ei
% \item LatentDirichletAllocation(n\_components=a, doc\_topic\_prior=b,\newline topic\_word\_prior=c,
%                                   learning\_decay=d,
%                                   learning\_offset=e,batch\_size=f)
%     \bi
%     \item a, b, c = randint(10, 50), randuniform(0, 1),  randuniform(0, 1)
%     \item d, e  = randuniform(0.51, 1.0), randuniform(1, 50), 
%     \item f = randchoice([150,180,210,250,300])
%     \ei
% \ei 


%  \\\hline
 \end{tabular}

\end{table}

==> texputback.tex <==
In the context of Marcus's comments, it is apropos to observe that there are several recent documented examples in SE where DL
did  not work better than alternate methods:
  \bi
  \item 
  When
 learning language models from source code.
Hellendoorn  et al. say that DL did not perform better   existing approaches~\cite{hellendoorn2017deep};
\item
For finding similar StackOverflow questions, Majumder et al. report that comparable results to DL can be achieved via hyperparameter optimization, three orders of magnitude faster~\cite{menzies2018500};
\item
For predicting slow runtimes in cloud computing,
Chen et al. applied neural and non-neural methods~\cite{chen2019predicting}. For that application, Chen et al      preferred   non-neural decision trees that performed (very slightly) worse than neural methods, but gave engineers more insight into what was causes the problems.  
\ei


In this section, we present the experimental results to answer the four research questions formulated in Section~\ref{sec:introduction}.

\begin{RQ}
{\bf RQ1.} What's 
the baseline method in this paper?
% the prior state of the art?
\end{RQ}

For RQ1, three commonly used conventional classifiers (\textit{Random Forest, Decision Tree} and \textit{Support Vector Machine with RBF kernal}) and DODGE~\cite{agrawal2019dodge} are used as the baseline methods. \textit{Random Forest, Decision Tree} and \textit{Support Vector Machine} are widely utilized in SE tasks due to their merits like low computing cost and highly robustness for performance on average. In this paper, our baseline is implemented with a weighted strategy in Scikit-learning \footnote{https://scikit-learn.org/stable/}, a popular Python package integrating a wide range of state-of-the-art machine learning algorithms.  DODGE proposed by Agrawal et al.~\cite{agrawal2019dodge} is a novel hyperparameter optimizer which can both achieve better performance than recent prominent defect prediction and hyperparameter optimization
results~\cite{fu2016tuning, ghotra2015revisiting} and reduce the computational cost in tuning by ignoring redundant tunings. Therefore, DODGE can be seen as a state-of-the-art method in hyperparameter optimization.
More specific technical details about DODGE have been exhaustively demonstrated in Section~\ref{sec:dodge}.

\begin{RQ}
{\bf RQ2.} 
For classifying imbalanced static code warnings, does deep learning succeed better than the prior state-of-the-art?
% Are deep neural networks better way to cope with imbalanced problem? (Comparison with traditional state-of-the-art)
\end{RQ}



 
% , however, since Cohen advises that 

% Note how, in these results, deep learning is often the winner. 

% Tables \ref{table:recall}, \ref{table:faslealarm}, \ref{table:AUC}, and \ref{table:runningcost} show our results. The columns in these table are sorted on the median recall of the different learning schemes (so all tables share the same column sort order).

% Before answering our research questions, we first comment on some
%   obvious effects:


% % \begin{table}[!b]
% % \caption{Summary of recall. The red cells show results which are better than
% % DNN\_weighted by more than a small effect size.}
% % % \small
% % \footnotesize
% % % \begin{adjustbox}{max width=0.48\textwidth}
% % \begin{tabular}{@{}llllllll@{}}
% % \hline
% % \multicolumn{1}{l}{}  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & CNN & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & \begin{tabular}[c]{@{}c@{}}SVM\_\\ RBF\end{tabular} \\ \hline
% %   Derby & 98 & 96 & {\color[HTML]{333333} 88} & 93 & 76 & 70 & 0 \\
% %  Mvn & 96 & 85 & 93 & 93 & 75 & 96 & 0 \\
% %  Lucence & 95 & 85 & 94 & 86 & \colorbox{Thistle}{97} & \colorbox{Thistle}{97} & 0 \\
% %  Phoenix & 98 & 95 & 76 & 87 & 85 & 90 & 0 \\
% %  Cass & 79 & 95 & \colorbox{Thistle}{93} & 68 & \colorbox{Thistle}{85} & \colorbox{Thistle}{90} & 0 \\
% %  Jmeter & 97 & 93 & 94 & 90 & \colorbox{Thistle}{98} & 94 & 0 \\
% %  Tomcat & 97 & 96 & 93 & 95 & 96 & 93 & 0 \\
% %  Ant & 89 & 88 & 88 & 83 & 81 & 87 & 0 \\
% %  Commons & 92 & 91 & 83 & 77 & 67 & \colorbox{Thistle}{95} & 0 \\ \hline
% %  Median & 96 & 91 & 89 & 86 & 84 & 90 & 0 \\  \hline
% % \end{tabular}
% % % \end{adjustbox}
% % \label{table:recall}
% % \end{table} 
% %  % Please add the following required packages to your document preamble:
% % % \usepackage{multirow}
% % % \usepackage[table,xcdraw]{xcolor}
% % % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% % \begin{table}[]
% % \caption{Summary of recall.}
% % % \small
% % \footnotesize
% % % \begin{adjustbox}{max width=0.48\textwidth}
% % \begin{tabular}{ccccccc}
% % \hline
% % \multicolumn{1}{l}{}  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & SVM\_RBF \\ \hline
% %   Derby & 98 & {\color[HTML]{333333} 88} & 93 & 76 & 70 & 0 \\
% %  Mvn & 96 & 93 & 93 & 75 & 96 & 0 \\
% %  Lucence & 95 & 94 & 86 & \colorbox{Thistle}{97} & \colorbox{Thistle}{97} & 0 \\
% %  Phoenix & 98 & 76 & 87 & 85 & 90 & 0 \\
% %  Cass & 79 & \colorbox{Thistle}{93} & 68 & \colorbox{Thistle}{85} & \colorbox{Thistle}{90} & 0 \\
% %  Jmeter & 97 & 94 & 90 & \colorbox{Thistle}{98} & 94 & 0 \\
% %  Tomcat & 97 & 93 & 95 & 96 & 93 & 0 \\
% %  Ant & 89 & 88 & 83 & 81 & 87 & 0 \\
% %  Commons & 92 & 83 & 77 & 67 & \colorbox{Thistle}{95} & 0 \\ \hline
% %  Average & 93 & 89 & 86 & 84 & 90 & 0 \\  \hline
% % \end{tabular}
% % % \end{adjustbox}
% % \label{table:recall}
% % \end{table} %  % Please add the following required packages to your document preamble:
% % % \usepackage{multirow}
% % % \usepackage[table,xcdraw]{xcolor}
% % % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% % \begin{table}[]
% % \caption{Summary of false alarm.}
% % % \small
% % \footnotesize
% % % \begin{adjustbox}{max width=0.48\textwidth}
% % \begin{tabular}{ccccccc}
% % \hline
% % \multicolumn{1}{l}{}  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & SVM\_RBF \\ \hline
% %   Derby & 0 & {\color[HTML]{333333} 1} & 0 & 0 & 0 & 0 \\
% %   Mvn & 0 & 1 & 0 & 0 & 0 & 0 \\
% %   Lucence & 8 & 4 & 4 & 1 & 1 & 0 \\
% %   Phoenix & 3 & 1 & 2 & 1 & 1 & 0 \\
% %   Cass & 0 & 2 & 0 & 0 & 0 & 0 \\
% %   Jmeter & 3 & 2 & 1 & 0 & 0 & 0 \\
% %   Tomcat & 3 & 3 & 1 & 0 & 0 & 0 \\
% %   Ant & 0 & 1 & 0 & 0 & 0 & 0 \\
% %  Commons & 7 & 1 & 1 & 0 & 0 & 0 \\ \hline
% % \end{tabular}
% % % \end{adjustbox}
% % \label{table:faslealarm}
% % \end{table}

% % \begin{table}[!t]
% % \caption{Summary of false alarm. There are no red cells in this table since no was better than
% % DNN\_weighted by more than a small effect size.}
% % % \small
% % \footnotesize
% % % \begin{adjustbox}{max width=0.48\textwidth}
% % \begin{tabular}{@{}llllllll@{}}
% % \hline
% % \multicolumn{1}{l}{}  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & CNN & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & \begin{tabular}[c]{@{}c@{}}SVM\_\\ RBF\end{tabular} \\ \hline
% %   Derby & 0 & 1 & {\color[HTML]{333333} 1} & 0 & 0 & 0 & 0 \\
% %   Mvn & 0 & 1 & 1 & 0 & 0 & 0 & 0 \\
% %   Lucence & 8 & 6 & 4 & 4 & 1 & 1 & 0 \\
% %   Phoenix & 3 & 3 & 1 & 2 & 1 & 1 & 0 \\
% %   Cass & 0 & 7 & 2 & 0 & 0 & 0 & 0 \\
% %   Jmeter & 3 & 4 & 2 & 1 & 0 & 0 & 0 \\
% %   Tomcat & 3 & 3 & 3 & 1 & 0 & 0 & 0 \\
% %   Ant & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\
% %  Commons & 7 & 0 & 1 & 1 & 0 & 0 & 0 \\ \hline
% %  Median & 3 & 3 & 2 & 1 & 0 & 1 & 0 \\  \hline
% % \end{tabular}
% % % \end{adjustbox}
% % \label{table:faslealarm}
% % \end{table}

% % % Please add the following required packages to your document preamble:
% % % \usepackage{multirow}
% % % \usepackage[table,xcdraw]{xcolor}
% % % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% % \begin{table}[]
% % \caption{Summary of AUC.}
% % % \small
% % \footnotesize
% % % \begin{adjustbox}{max width=0.48\textwidth}
% % \begin{tabular}{ccccccc}
% % \hline
% % \multicolumn{1}{l}{}  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & SVM\_RBF \\ \hline
% %  Derby & 100 & {\color[HTML]{333333} 91} & 100 & 100 & 85 & 50 \\
% %   Mvn & 100 & 91 & 100 & 99 & 98 & 50 \\
% %   Lucence & 98 & 93 & 98 & 100 & 97 & 50 \\
% %   Phoenix &100 & 89 & 99 & 99 & 94 & 50 \\
% %   Cass & 99 & 90 & 99 & 100 & 95 & 50 \\
% %   Jmeter & 99 & 95 & 96 & 100 & 97 & 50 \\
% %   Tomcat & 100 & 91 & 100 & 100 & 96 & 50 \\
% %   Ant & 100 & 94 & 100 & 99 & 93 & 50 \\
% %  Commons & 98 & 90 & 100 & 100 & 97 & 50 \\ \hline
% % \end{tabular}
% % % \end{adjustbox}
% % \label{table:AUC}
% % \end{table}

% % \begin{table} 
% % \caption{Summary of AUC. There are no red cells in this table since no was better than
% % DNN\_weighted by more than a small effect size.}
% % % \small
% % \footnotesize
% % % \begin{adjustbox}{max width=0.48\textwidth}
% % \begin{tabular}{@{}llllllll@{}}
% % \hline
% % \multicolumn{1}{l}{}  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & CNN & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & \begin{tabular}[c]{@{}c@{}}SVM\_\\ RBF\end{tabular} \\ \hline
% %  Derby & 100 & 99 & {\color[HTML]{333333} 91} & 100 & 100 & 85 & 50 \\
% %   Mvn & 100 & 99 & 91 & 100 & 99 & 98 & 50 \\
% %   Lucence & 98 & 97 & 93 & 98 & 100 & 97 & 50 \\
% %   Phoenix &100 & 99 & 89 & 99 & 99 & 94 & 50 \\
% %   Cass & 99 & 98 & 90 & 99 & 100 & 95 & 50 \\
% %   Jmeter & 99 & 97 & 95 & 96 & 100 & 97 & 50 \\
% %   Tomcat & 100 & 99 & 91 & 100 & 100 & 96 & 50 \\
% %   Ant & 100 & 99 & 94 & 100 & 99 & 93 & 50 \\
% %  Commons & 98 & 99 & 90 & 100 & 100 & 97 & 50 \\ \hline
% %  Median & 99 & 98 & 92 & 99 & 100 & 95 & 50 \\  \hline
% % \end{tabular}
% % % \end{adjustbox}
% % \label{table:AUC}
% % \end{table}

% % % Please add the following required packages to your document preamble:
% % % \usepackage{booktabs}
% % % \usepackage{multirow}
% % % \usepackage[table,xcdraw]{xcolor}
% % % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% % \begin{table}[]
% % \caption{Summary of running time(Second/per iteration).}
% % % \small
% % \footnotesize
% % % \begin{adjustbox}{max width=0.48\textwidth}
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% %  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & SVM\_RBF \\ \midrule
% %   Derby & 16.3 & {\color[HTML]{333333} 69.1} & 18.1 & 5.1 & 4.9 & 17.4 \\
% %   Mvn & 9.7 & 138.4 & 10.1 & 1.8 & 1.7 & 3.3 \\
% %   Lucence & 24.2 & 241.8 & 24.3 & 7.6 & 6.8 & 28.2 \\
% %   Phoenix & 20.3 & 235.5 & 20.5 & 4.5 & 4.4 & 13.9 \\
% %   Cass & 20.3 & 174.3 & 25.3 & 5.3 & 5.1 & 15.5 \\
% %   Jmeter & 12.7 & 65.5 & 12.3 & 1.7 & 1.6 & 3.2 \\
% %   Tomcat & 17.8 & 89.5 & 17.6 & 2.9 & 2.8 & 7.7 \\
% %   Ant & 18.2 & 63.2 & 19.3 & 2.7 & 2.6 & 6.9 \\
% %  Commons & 16.8 & 40.5 & 17.8 & 1.4 & 1.3 & 2.6 \\ \bottomrule
% % \end{tabular}
% % % \end{adjustbox}
% % \label{table:runningcost}
% % \end{table}

% % % \begin{table}[!b]
% % % \caption{Summary of running time(Second/per training).}
% % % % \small
% % % \footnotesize
% % % % \begin{adjustbox}{max width=0.48\textwidth}
% % % \begin{tabular}{@{}llllllll@{}}
% % % \toprule
% % %  Dataset & \begin{tabular}[c]{@{}c@{}}DNN\_\\ weighted\end{tabular} & CNN & DODGE & DNN & \begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & \begin{tabular}[c]{@{}c@{}}SVM\_\\ RBF\end{tabular} \\ \midrule
% % %   Derby & 16.3 & 86.7 & 69.1 & 18.1 & 5.1 & 4.9 & 17.4 \\
% % %   Mvn & 9.7 & 50.2 & 138.4 & 10.1 & 1.8 & 1.7 & 3.3 \\
% % %   Lucence & 24.2 & 95.7 & 241.8 & 24.3 & 7.6 & 6.8 & 28.2 \\
% % %   Phoenix & 20.3 & 76.8 & 235.5 & 20.5 & 4.5 & 4.4 & 13.9 \\
% % %   Cass & 20.3 & 98.4 & 174.3 & 25.3 & 5.3 & 5.1 & 15.5 \\
% % %   Jmeter & 12.7 & 23.2 & 65.5 & 12.3 & 1.7 & 1.6 & 3.2 \\
% % %   Tomcat & 17.8 & 38.1 & 89.5 & 17.6 & 2.9 & 2.8 & 7.7 \\
% % %   Ant & 18.2 & 68.2 & 63.2 & 19.3 & 2.7 & 2.6 & 6.9 \\
% % %  Commons & 16.8 & 93.4 & 40.5 & 17.8 & 1.4 & 1.3 & 2.6 \\ \hline
% % %   Average & 17.6 & 70.1 & 124.2 & 18.4 & 3.7 & 3.5 & 10.9 \\  
% % %   \bottomrule
% % % \end{tabular}
% % % % \end{adjustbox}
% % % \label{table:runningcost}
% % % \end{table}




% % \bi
% % \item
% % SVM performed very badly, possibly due to a very poor choice of kernel.  
% % \item
% % Weighted\_DNN had largest recalls.
% % \item 
% % In terms of false alarms and AUC, with the exception of SVM, there were no treatments performing more than a small effect better than Weighted\_DNN.
% % \item
% % For recall, sometimes, the untuned non-DL learners performed better than Weighted\_DNN 
% % (see the red cells in Table~\ref{table:recall}). But when those learners peformed badly,
% % they performed very badly indeed. The Weighted\_DNN recalls were 
% % \[79,89,92,95,96,97,97,98,98\]
% % while the (say) Random Forest recall results were
% % \[67,75,76,81,85,85,96,97,98\]. That is, overall,
% % we cannot rely on the the non-DL learners to produce better models.
% % \item
% % Also, for recall, the DL methods all had similar performance (as assessed via Cohen's $\Delta$).
% % Still, we might prefer Weighed\_DNN since it has the highest median performance.
% % \item
% % For runtimes, the DNN variants were faster than CNN.
% % \item
% % For runtimes, the DNN variants were far faster than 
% % the DODGE hyperparameter optimizer (18 seconds versus 124 seconds).
% % \ei
% % Turning now to the research questions:
% % \begin{RQ}
% % {\bf RQ1.} 
% % Is DL relatively better at  recognizing actionable static code warnings?
% % % the prior state of the art?
% % \end{RQ}
% % Looking over Tables \ref{table:recall}, \ref{table:faslealarm}, \ref{table:AUC} and \ref{table:runningcost}, we see that un-tuned SVM performed worst.
% % Measured in terms of false alarm and AUC, most of the methods are equal.
% % Measured in terms of recall, Weighted\_DNN has the best median performance and a much higher median performance than the untuned non-DL learners.
% % Measured in terms of runtime, DNN ran faster than CNN and much faster than 
% % the DODGE hyperparameter optimizer.
% % Hence, overall, we say that
% % \bi
% % \item
% % Untuned non-DL learners like decision trees work worst;
% % \item
% % Those learners, plus hyperparameter optimization, work better;
% % \item
% % But the DL method called Weighted\_DNN works best of all (similar performance scores, must faster runtime).
% % \ei


% % \begin{RQ}
% % {\bf RQ2.} 
% % Is DL training very slow for recognizing actionable static code warnings?
% % % the prior state of the art?
% % \end{RQ}
% % Looking at Table~\ref{table:runningcost}, 
% % we see that   no learning scheme seemed slow enough to require specialized hardware such as cloud-based GPUs.  
% % As shown in that table,
% % the computational cost for \textit{DNN\_weighted} and \textit{DNN} are much slow as expected, about 3 to 13 times slower compared with traditional classifiers, like \textit{Decision Tree} and \textit{Random Forest}. Moreover, compared with the runtime of \textit{Support Vector Machine with RBF kernel}, \textit{DNN} models only outperforms \textit{SVM} in one case (Lucence), and is beaten by RBF kernel \textit{SVM} in most datasets. 
% % That said, by implementing a simple framework of DNN model with linear activation function and adopting early stopping strategy, our computational cost is not that excessively slow in contrast with previous runtime comparison. 
% % %Fu et al.~\cite{fu2017easy} report tuning SVM with DE (differential evolution~\cite{storn1997differential}) can achieve better performance than than \textit{CNN} with 84 times faster running cost. 
% % \textit{DODGE} is the most computational-high one in the six methods since it runs SMOTE many times to assess different parameter settings.


% % In summary, in this domain,  the extra running overhead of  deep learning
% % is more compensated by the significant performance improvement.



% \begin{RQ}
% {\bf RQ3.} 
% Why is DL so fast in this domain?
% % the prior state of the art?
% \end{RQ}
% DL is not usually as fast as seen here. For example, average training times
% for some high dimensional visual processing problem (e.g. for autonomous cars)
% cane be days to weeks.
% So what is so special about 
% recognizing actionable static code warnings?


% We conjecture, DL was so fast here since our problems is {\em not} inherently high dimensional? To test that, we applied the  Equation~\ref{eq:cr} to our none data sets to generate
% Table~\ref{table:dimensionality_L1},
% While our data sets have 39 to 60 attributes, the Levina et al. calculator reported that the median intrinsic dimensionality of our data had median values of just 0.93. Hence, it is hardly surprising the DL ran so fast for recognizing static code warnings since this task is intrinsically very simple.

 
% Going forward, this could mean that DL might be especially useful, and easy to apply, to SE problems with inherently low dimensionality. This could be a fruitful area for future research.
% Gong et al.~\cite{gong2019intrinsic} report 512-dim image data can be efficiently converted into lower space with intrinsic dimension less than 20. Moreover, a visual validation are
% provided by mapping a 3-dim data into 2-dim by a deep neural network based non-linear mapping method called DeepMDS~\cite{gong2019intrinsic}.
 


% To answer this research question, we employ Keras to implement a DNN model. To be specific, our DNN model contains 5 layers and 30 neurons for each hidden layers. And the Relu is utilized as activation functions of each hidden layer. Relu represents a rectified linear unit, whose formula denoted as $ f(x) = max(0, x) $. It is the most commonly used activation function in deep learning, especially for CNN models. As a universal choice of various activation functions, Relu is known for many merits like fast to compute and converge in practice and its gradients not vanishing when $ x > 1$ holds or the current neuron is activated. Since actionable warning identification is a binary problem, for any instance $ i $ of warnings, its label $ y_i \in\{0, 1\} $, where $ 0 $ denotes this warning is unactionable and $ 1 $ denotes as actionable. Consequently, we use softmax as the activation function for the output of our network in the output layer. Softmax takes the vectors generated from last hidden layer as inputs and proceeds them by exponentiatial operation with a power of $e$ and mapping it into a list of probability distribution of all the label class candidates. For each instance, the list of Softmax vector $ [P_0, P_1] $ generated from softmax function always sums to 1, where $ P_0$ is the probability that this bug is unactionable while $ P_1$ denoted as actionable. And the probability list of each unlabeled instance generated by the deep neural network can be employed to predict its label and calculate the cross entropy. Softmax also works for multi-label classification problem, the formula is defined as follows:

% \[ P_i =
% Softmax(y_i)
% \frac{e^{y_i}}{\sum_{j=1}^N e^{y_i}}   \]
% \[where: \sum_{i=1}^N P_i = 1\]
    

% To address the data imbalance problem, a weighted strategy is employed for \textit{DNN\_weighted} model. To be specific, we weight up the minority class, actionable class, proportionally since it's highly underrepresented. The mechanism of weighted strategy is to utilize reciprocal of the ratio for class 0 and 1 to weight the loss function during  the training phase, so that the pattern of minority class is learned equally as majority.
% There are also some other strategies to cope with data imbalance problem, like duplicate instances of minority class and fed them to classifiers. However, reusing many copies of one instance in the training set causes the over-fitting problem~\cite{shalev2014understanding} and extra computational cost.

% The experiment results (Recall, False alarm and AUC) are reported in Table~\ref{table:recall}, Table~\ref{table:faslealarm} and Table~\ref{table:AUC} respectively. Each of the table reports the median value of ten runs. Based on the results shown in Table~\ref{table:recall}, it can be observed that \textit{DNN\_wighted} outperforms other baselines in term of recall in 6 test cases (Derby, Mvn, Phoenix, Jmeter, Tomcat and Ant), and in one datasets (Lucence), there is not significant difference between \text{DNN\_weighted} and the winner in baseline. The violation where baseline perform better than \textit{DNN\_wighted} is highlighted in \colorbox{Thistle}{purple}. Moreover, according to Table~\ref{table:recall}, the average of recall on nine projects shows \textit{DNN\_weighted} beats other approaches in evidence. Besides, as respect to false alarm and AUC summarised in Table\ref{table:faslealarm} and Table\ref{table:AUC}, results of \textit{DNN\_weighted} don't show significant difference with other approaches, except from the worst method, \textit{SVM\_RBF}.



% \begin{RQ}
% {\bf RQ3.}
% Does deep learning models need long training time?
% % What's the computational cost compared with conventional machine learning algorithms and the state-of-the-art? 
% \end{RQ}


% Table~\ref{table:runningcost} shows the average running time(/second) of ten repeats for six learners. All of the experiments are performed on GPU GeForce GTX 1080 with RAM 8GB. Since deep neural networks are defined as high computational methods in previous literature~\cite{fu2017easy}, it's essential to compare the runtimes of different approaches to validate if the high cost of computation overhead worth the improved performance.



% \begin{table}[!t]
% \caption{Summary of dimensionality of nine datasets.
% Calculated using Equation~\ref{eq:cr}.}
% % \small
% \footnotesize
% % \begin{adjustbox}{max width=0.48\textwidth}
% \begin{tabular}{@{}cccc@{}}
% \toprule
% \multicolumn{1}{l}{}  Dataset & \begin{tabular}[c]{@{}c@{}}original\\ dimensionality\end{tabular} & \begin{tabular}[c]{@{}c@{}}intrinsic \\ dimensionality\end{tabular} & \begin{tabular}[c]{@{}c@{}}instance \\ counts\end{tabular} \\ \midrule

%   Lucence & 57 & \colorbox{Apricot}{0.22} & 3259 \\
  
%  Commons & 39 & \colorbox{Apricot}{0.75} & 725 \\ 
%   Phoenix & 44 & \colorbox{Apricot}{0.80} & 2235 \\
  
%   Ant & 56 & \colorbox{Apricot}{0.82} & 1229 \\
%   Derby & 58 & \colorbox{Apricot}{0.93} & 2479 \\
  
%   Tomcat & 60 & \colorbox{Apricot}{0.95} & 1435 \\
%   Mvn & 47 & \colorbox{Apricot}{1.10} & 813 \\
  
%   Jmeter & 49 & \colorbox{Apricot}{1.25} & 604 \\
  
%   Cass & 55 & \colorbox{Apricot}{1.94} & 2584 \\\bottomrule
% \end{tabular}
% % \end{adjustbox}
% \label{table:dimensionality_L2}
% \end{table}

 

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \caption{Summary of statistical results of recall, false alarm, AUC and running time of 5 classifiers on nine projects. (cross validation VS cross versions)}
% \footnotesize
% \begin{adjustbox}{max width=0.48\textwidth}
% \begin{tabular}{|l|c|l|l|l|l|l|l|}
% \hline
% Metrics & \multicolumn{1}{l|}{Evaluation} & \begin{tabular}[c]{@{}l@{}}Statistical\\ test\end{tabular} & \begin{tabular}[c]{@{}l@{}}DNN\\ \_weighted\end{tabular} & CNN & \begin{tabular}[c]{@{}l@{}}Random\\ Forest\end{tabular} & \begin{tabular}[c]{@{}l@{}}Decision\\ Tree\end{tabular} & \begin{tabular}[c]{@{}l@{}}SVM\\ \_RBF\end{tabular} \\ \hline
% \multirow{4}{*}{recall} & \multirow{2}{*}{5 by 5} & median & 0.03 & 0.33 & 0.79 & 0.89 & 0.00 \\ \cline{3-8} 
%  &  & IQR & 0.40 & 0.00 & 0.22 & 0.05 & 0.00 \\ \cline{2-8} 
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}cross\\ version\end{tabular}} & median & 0.96 & 0.93 & 0.85 & 0.93 & 0.00 \\ \cline{3-8} 
%  &  & IQR & 0.05 & 0.05 & 0.20 & 0.07 & 0.00 \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}fasle \\ alarm\end{tabular}} & \multirow{2}{*}{5 by 5} & median & 0.03 & 0.33 & 0.00 & 0.01 & 0.00 \\ \cline{3-8} 
%  &  & IQR & 0.30 & 0.01 & 0.01 & 0.02 & 0.00 \\ \cline{2-8} 
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}cross\\ version\end{tabular}} & median & 0.03 & 0.01 & 0.00 & 0.03 & 0.00 \\ \cline{3-8} 
%  &  & IQR & 0.03 & 0.01 & 0.00 & 0.03 & 0.00 \\ \hline
% \multirow{4}{*}{AUC} & \multirow{2}{*}{5 by 5} & median & 0.50 & 0.50 & 0.99 & 0.93 & 0.50 \\ \cline{3-8} 
%  &  & IQR & 0.01 & 0.06 & 0.00 & 0.03 & 0.00 \\ \cline{2-8} 
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}cross\\ version\end{tabular}} & median & 1.00 & 0.99 & 1.00 & 0.96 & 0.50 \\ \cline{3-8} 
%  &  & IQR & 0.01 & 0.01 & 0.01 & 0.03 & 0.00 \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}running\\ time\end{tabular}} & \multirow{2}{*}{5 by 5} & median & 32.24 & 76.94 & 4.32 & 3.14 & 11.30 \\ \cline{3-8} 
%  &  & IQR & 31.59 & 82.33 & 3.91 & 3.40 & 21.49 \\ \cline{2-8} 
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}cross\\ version\end{tabular}} & median & 17.80 & 76.80 & 2.90 & 2.80 & 7.70 \\ \cline{3-8} 
%  &  & IQR & 4.00 & 43.20 & 3.30 & 3.20 & 12.20 \\ \hline
% \end{tabular}
% \end{adjustbox}
% \label{table:statistical}
% \end{table}


% \begin{algorithm}
% \SetAlgoLined
% \KwResult{}
% \KwResult{Write here the result }
%  Import data from \texttt{Testdata.py};
%  \input{}
%  \While{While condition}{
%   instructions\;
%   \eIf{condition}{
%   instructions1\;
%   instructions2\;
%   }{
%   instructions3\;
%   }
%  }
%  \caption{Pseudo Code for Intrinsic Dimension by Box-counting}
%  \label{alg:intrinsic1}
% \end{algorithm}

% To answer this research question, we simulate four randomly generated high-dimensional datasets with size of instances $ s = 1000 $ and dimensionality $ dim = $ 5, 10, 20, 40 respectively by Gaussian distribution. We further employ Box-counting~\cite{camastra2003data} method to condense the dimensionality of randomly generated date. Figure~\ref{fig:random} reports the curve of $ln (C_m(r)) $ against $ln(r) $. This fractal method estimates the intrinsic dimensionality by accessing the maximum gradient of the curve. The intrinsic dimensionality obtained by four simulated datasets are reported as 3.4, 5.3, 10.3 and 13.4 respectively.
% Courtney et al.~\cite{courtney1993shotgun} claim that there exists correlations among randomly generated data.
% % we utilize Gaussian distribution to randomly generate high-dimensional datasets with 1000 data instances. 

% 9 SE datasets are further evaluated by this approach, and the original dimension and intrinsic dimension counts are reported and highlighted in \colorbox{Apricot}{orange} in Table~\ref{table:dimensionality}. In contract with randomly generated datasets, SE data are much more condensed. Since the golden set of features are further extracted into different segments, the original dimension counts of different projects are various.
% As shown in Table~\ref{table:dimensionality}, the conclusion can be drawn that warning features extracted from nine static projects are just embedded into high dimensional space, they can be converted into much more condensed space. Therefore, before using any high dimensional methods, we have to cast doubt on whether our seemingly complex data is just embedded in a high dimensional space and whether the methods are necessarily feasible only for high dimensional data. 


==> texrelated.tex <==


\section{Why Study DL?}

To say the least,
 there has been much recent interest
 in the application
 of deep learning (DL) neural
 networks in software engineering.
Applications for DL incldue bug localization~\cite{huo2019deep}, sentiment analysis~\cite{lin2018sentiment}, code clone detection~\cite{white2016deep}, etc.
Yet some researchers are worried that DL is being applied with insufficient critical assessment. 
For example,  Gary Marcus~\cite{marcus2018deep} 
 warns than DL may be so over-hyped
that it runs  ``fresh risk for seriously dashed expectations'' that could blinker AI researchers from trying new ideas as well as
bringing  another AI winter (the period in the mid to late 1980s when most AI companies went bankrupt due to poor generalization
of their methods).

Also, numerous researchers at a recent United States National Science Foundation (NSF) meeting on high performance computing~\cite{nsf20} issued warnings about the hardware requirements for DL.
When training a DL, the same data must be run through its networks in thousands of ``epochs'' where, each time, the DL fine tunes its internal weights. This is a slow process that can require much time and much expensive hardware
(which may not be widely available). Also, the hardware used to optimize DL is evolving so rapidly that   in a  mere matter of months, older solutions may no longer be operational.  Hence, results using
DL-based analytics can be hard to commission,
hard to maintain, and hard to reproduce.


\textit{Auto-encoder}
%
aims to minimize the difference (e.g., cross-entropy loss) between the input and output layers by network parameter optimization. The optimization is usually conducted by a layer-to-layer pre-training and a global parameter optimization with the training sets. In SE studies, Auto-encoder is regarded as an unsupervised tool for feature reduction, namely transforming high-dimensional initial input vectors into low-dimensional ones (hidden layers).
%

% \textbf{GAN(Generative Adversarial Networks)}

% \textbf{Deep Reinforcement Learning}
 
